Learning to Infer Generative Template Programs for Visual Concepts

People grasp flexible visual concepts from a few examples. We explore a neurosymbolic system that learns how to infer programs that capture visual concepts in a domain-general fashion. We introduce Template Programs: programmatic expressions from a domain-specific language that specify structural and parametric patterns common to an input concept. Our framework supports multiple concept-related tasks, including few-shot generation and co-segmentation through parsing. We develop a learning paradigm that allows us to train networks that infer Template Programs directly from visual datasets that contain concept groupings. We run experiments across multiple visual domains: 2D layouts, Omniglot characters, and 3D shapes. We find that our method outperforms task-specific alternatives, and performs competitively against domain-specific approaches for the limited domains where they exist.

==> algorithms/finetune.tex <==
\begin{algorithm}[H]
   \caption{Bootstrapped Finetuning}
   \label{alg:finetune}
%   \textbf{Input:}~\infnets,~\Target,~\Executor,~\Objective \\
%    \textbf{Output:}~\infnets~fine-tuned on~\Target ~
    \begin{algorithmic}
%        \STATE \gennets~=~copy(\infnets) 
        \FOR{$\text{outer-loop rounds}$}
        \MYCOMMENT{Infer template concepts and instantiations}
        \STATE \text{inf\_data} = \textit{inferConcepts}(\infnets, \Target)
        \MYCOMMENT{Construct data triplets from inferred data}
        \STATE \text{st\_data} = \text{[}(\VisGroup,~\TemplateGroup,~\ProgramGroup)~$\forall$~(\VisGroup,~\TemplateGroup,~\ProgramGroup)$\in$~\text{inf\_data]}
        \STATE \text{lest\_data} = \text{[}((\Executor(\program) $\forall$ \program $\in$ \ProgramGroup),~\TemplateGroup,~\ProgramGroup)
        \STATE ~~~~ $\forall$~(\_,~\TemplateGroup,~\ProgramGroup)~$\in$~\text{inf\_data]}
        \STATE \textit{trainGenerative}(\gennets,  \text{inf\_data})
        \STATE \text{ws\_data} = \textit{sampleConcepts(\gennets)}
        \MYCOMMENT{Finetune inference networks}
        \FOR{$\text{inner-loop rounds}$}
        \STATE \text{batch\_data} = \textit{sampleBatch}(
        \STATE ~~~~random.choice(\text{[st\_data, lest\_data, ws\_data]}))
        \STATE \textit{MLUpdate}(\infnets, \text{batch\_data})
        \ENDFOR
        \ENDFOR
    \end{algorithmic}
\end{algorithm}


==> algorithms/infer_concepts.tex <==
\begin{algorithm}[H]
   \caption{inferConcepts}
   \label{alg:inferconcepts}
    \begin{algorithmic}
        \STATE data = []
        \FOR{\VisConcept $\in$ \Target}
        \STATE \VisGroup = \textit{subSample}(\VisConcept, \text{group\_size})
        \MYCOMMENT{Search for Template Program that optimizes \Objective}
        \STATE \TemplateGroup,~\ProgramGroup = \textit{beamSearch}(\VisGroup, \infnets, \Objective)
        \STATE data.append((\VisGroup,~\TemplateGroup,~\ProgramGroup))
        \ENDFOR
        \STATE return data
    \end{algorithmic}
\end{algorithm}


